Cognitive Constructivism and the Epistemic Significance of Sharp Statistical Hypotheses in Natural Sciences

This book presents our case in defense of a constructivist epistemological framework and the use of compatible statistical theory and inference tools. The basic metaphor of decision theory is the maximization of a gambler's expected fortune, according to his own subjective utility, prior beliefs an learned experiences. This metaphor has proven to be very useful, leading the development of Bayesian statistics since its XX-th century revival, rooted on the work of de Finetti, Savage and others. The basic metaphor presented in this text, as a foundation for cognitive constructivism, is that of an eigen-solution, and the verification of its objective epistemic status. The FBST - Full Bayesian Significance Test - is the cornerstone of a set of statistical tolls conceived to assess the epistemic value of such eigen-solutions, according to their four essential attributes, namely, sharpness, stability, separability and composability. We believe that this alternative perspective, complementary to the one ofered by decision theory, can provide powerful insights and make pertinent contributions in the context of scientific research.

==> ARVI.TEX <==

 %\mbox{} 
   
 {\large 
 %\resizebox{6.5in}{6.5in}{ 
 \[
 \dgARROWPARTS=12 
 \begin{diagram}
 \node[2]{\Ovalbox{1}} 
 \arrow{se,t}{5} \arrow{sw,t}{6} \arrow[4]{s,r,8,<>}{4} \\ 
 \node{\Ovalbox{3}} \arrow[2]{e,t,4,-}{21} \arrow[2]{s,l,<>}{3} 
  \arrow[2]{se,t,2}{19}  \arrow{ssse,t,4}{16}
 \node[2]{\Ovalbox{2}}  \arrow[2]{s,r,<>}{2} 
  \arrow[2]{sw,t,2}{7}   \arrow{sssw,t,4}{9} \\ 
  \node[2]{\ovalbox{0}} \\ 
 \node{\Ovalbox{5}} \arrow[2]{e,t,5,-}{1} \arrow[2]{s,l,<>}{17} 
  \arrow{se,b}{18}   
 \node[2]{\Ovalbox{4}} \arrow[2]{s,r,<>}{11}  \arrow{sw,b}{8} \\ 
 \node[2]{\Ovalbox{6}} \arrow[2]{s,r,9,<>}{20}    % \\ %  
                \arrow{se,t}{10} \arrow{sw,t}{15} \\ %
 \node{\Ovalbox{8}} \arrow[2]{e,t,3,-}{13} \arrow{se,b}{12}   
                                % \arrow{ne,t}{15}    %\arrow{sse,-,..} 
 \node[2]{\Ovalbox{7}} \arrow{sw,b}{14}            \\ % 
                                % \arrow{nw,t}{10} \\ %\arrow{ssw,-,..} \\ 
 \node[2]{\Ovalbox{9}} \arrow{s,r,<>}{22} \\ 
 \node[2]{\Ovalbox{10}} \\ 
 \end{diagram}
 \] 
 }%\Large 

 \mbox{} \vspace{-2.0cm} \mbox{} 

 \centerline{Figure JB.3: The Tree of Life, by Isaac Luria.} % (Ari).} 
 \centerline{A lattice diagram of 11 key concepts and 22 inter-connections.} 
 \centerline{\mbox{}} 
 \centerline{Free Allegoric Interpretation:} % (by an anonymous student):}  
 \centerline{1- Systemic Evolution, 2- Symmetry, 3- Quantization, 
             0- Language,}  
 \centerline{4- Precision, 5- Stability, 6- Eigen-Solution, 
             7- Composition,} 
 \centerline{8- Separation, 9- Recombination, 10- Individual Organism.}   


